Discovering Avoidable Planner Failures of Autonomous Vehicles using Counterfactual Analysis in Behaviorally Diverse Simulation

Automated Vehicles require exhaustive testing in simulation to detect as many safety-critical failures as possible before deployment on public roads. In this work, we focus on the core decision-making component of autonomous robots: their planning algorithm. We introduce a planner testing framework that leverages recent progress in simulating behaviorally diverse traffic participants. Using large scale search, we generate, detect, and characterize dynamic scenarios leading to collisions. In particular, we propose methods to distinguish between unavoidable and avoidable accidents, focusing especially on automatically finding planner-specific defects that must be corrected before deployment. Through experiments in complex multi-agent intersection scenarios, we show that our method can indeed find a wide range of critical planner failures.

==> references.tex <==
\begin{thebibliography}{00}
% General
\bibitem{driving_to_safety} N. Kalra, and S. M. Paddock, ``Driving to Safety: How Many Miles of Driving Would It Take to Demonstrate Autonomous Vehicle Reliability?'', Santa Monica, CA: RAND Corporation, 2016, https://www.rand.org/pubs/research\_reports/RR1478.html.
\bibitem{chainer} S. Tokui, R. Okuta, T. Akiba, Y. Niitani, T. Ogawa, S. Saito, S. Suzuki, K. Uenishi, B. Vogel, and H. Y. Vincent, ``Chainer: A Deep Learning Framework for Accelerating the Research Cycle'', Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining, 2019, pp.2002--2011.

% Traffic Simulator
\bibitem{carla} A. Dosovitskiy, G. Ros, F. Codevilla, A. Lopez, and V. Koltun, ``{CARLA}: {An} Open Urban Driving Simulator'', Proceedings of the 1st Annual Conference on Robot Learning, 2017, pp.1--16.
\bibitem{torcs} E. Espi\'e, C. Guionneau, B. Wymann, C. Dimitrakakis, R. Coulom, and A. Sumner, ``{TORCS}, The Open Racing Car Simulator'', \texttt{http://www.torcs.org}, 2005.
\bibitem{sumo} D. Krajzewicz, J. Erdmann, M. Behrisch, and L. Bieker, ``Recent Development and Applications of {SUMO - Simulation of Urban MObility}'', International Journal On Advances in Systems and Measurements, December, 2012.
\bibitem{coincar_sim} M. Naumann, F. Poggenhans, M. Lauer, and C. Stiller, ``{C}o{I}n{C}ar-{S}im: An Open-Source Simulation Framework for Cooperatively Interacting Automobiles'', Proceeding of IEEE Intelligent Vehicles Symposium (IV), 2018, pp.1879--1884.
\bibitem{fluids} H. Zhao, A. Cui, S. A. Cullen, B. Paden, M. Laskey, and K. Goldberg, ``FLUIDS: A First-Order Local Urban Intersection Driving Simulator'', in IEEE International Conference on Automation Science and Engineering, August, 2018.
\bibitem{common_road} M. Althoff, M. Koschi, and S. Manzinger, ``CommonRoad: Composable benchmarks for motion planning on roads'', Proceedings of the IEEE Intelligent Vehicles Symposium (IV), 2017, pp.719--726.
\bibitem{bicycle_model} P. Polack, F. Altch\'e, B. d'Andr
\'ea Novel, and A. de La Fortelle, ``The kinematic bicycle model: A consistent model for planning feasible
trajectories for autonomous vehicles?'', Proceedings of the IEEE Intelligent Vehicles Symposium (IV), 2017, pp.812--818.

% Diversity acquisition
\bibitem{social_gan} A. Gupta, J. Johnson, L. Fei-Fei, S. Savarese, and A. Alahi, ``Social GAN: Socially Acceptable Trajectories With Generative Adversarial Networks'', The IEEE Conference on Computer Vision and Pattern Recognition (CVPR), June, 2018, pp.2255--2264.
\bibitem{drogon} C. Choi, A. Patil, and S. Malla, ``{DROGON}: A Causal Reasoning Framework for Future Trajectory Forecast'', arXiv preprint arXiv:1908.00024, 2019.
\bibitem{diversity_aware_prediction} X. Huang, S. G. McGill, J. A. DeCastro, B. C. Williams, L. Fletcher, J. J. Leonard, and G. Rosman, ``Diversity-Aware Vehicle Motion Prediction via Latent Semantic Sampling'', arXiv preprint arXiv:1911.12736, 2019.
\bibitem{interaction_aware} Y. Hu, A. Nakhaei, M. Tomizuka, and K. Fujimura, ``Interaction-aware Decision Making with Adaptive Strategies under Merging Scenarios'', in IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), 2019.
\bibitem{microscpic_multi_agent_rl}, G. Bacchiani, D. Molinari, and M. Patander, ``Microscopic Traffic Simulation by Cooperative Multi-agent Deep Reinforcement Learning'', in International Conference on Autonomous Agents and Multiagent Systems (AAMAS), 2019.

\bibitem{fps} T. F. Gonzalez, ``Clustering to minimize the maximum intercluster distance'', Theoretical Computer Science, 1985, vol.38, pp.293--306.
% Do we need cite ``A Best Possible Heuristic for the k-Center Problem''?

% Trajectory distances, Evaluation metrics
% \bibitem{trajectory_clustering_survey} J. Bian, D. Tianb, Y Tang, and D. Tao, ``A survey on trajectory clustering analysis'', arXiv preprint arXiv:1802.06971, 2018.
\bibitem{dtw} D. J. Berndt, and J. Clifford, ``Using dynamic time warping to find patterns in time series'', in AAAI-94 Workshop of Knowledge Discovery in Databases (KDD), 1994, pp.359--370.
\bibitem{lcss} M. Vlachos, G. Kollois, and D. Gunopulos, ``Discovering Similar Multidimensional Trajectories'', Proceedings of the 18th International Conference on Data Engineering (ICDE), 2002, pp.673--684.
\bibitem{trajectory_measure_review} N. Magdy, M. A. Sakr, T. Mostafa, and K. El-Bahnasy, ``Review on Trajectory Similarity Measures'', in 2015 IEEE Seventh International Conference on Intelligent Computing and Information Systems (ICICIS), December, 2015.
\bibitem{trajectory_measure_review_2019} H. Su, S. Liu, B. Zheng, X. Zhou, and K. Zheng, ``A Survey of Trajectory Distance Measures and Performance Evaluation'', in the VLDB Journal, https://doi.org/10.1007/s00778-019-00574-9, 2019.
\bibitem{brownian_bridge} J. S. Horne, E. O. Garton, S. M. Krone, and J. S. Lewis, ``Analyzing Animal Movements Using Brownian Bridges'', in Ecology, vol.88, No. 9, 2007, pp.2354--2363.
\bibitem{mon_analysis} L. A. Thiede, and P. P. Brahma, ``Analyzing the Variety Loss in the Context of Probabilistic Trajectory Prediction'', arXiv preprint arXiv:1907.10178, 2019.

% Diversity score
\bibitem{dsgan} D. Yang, S. Hong, Y. Jang, T. Zhao, and H. Lee, ``Diversity-Sensitive Conditional Generative Adversarial Networks'', in the International Conference on Learning Representations (ICLR), 2019.
\bibitem{fid} M. Heusel, H. Ramsauer, T. Unterthiner, B. Nessler, and S. Hochreiter, ``GANs Trained by a Two Time-Scale Update Rule Converge to a Local Nash Equilibrium'', Advances in Neural Information Processing Systems 30, 2017, pp.6626--6637.
\bibitem{lpips} R. Zhang, P. Isola, A. A. Efros, E. Shechtman, and O. Wang, ``The Unreasonable Effectiveness of Deep Features as a Perceptual Metric'', The IEEE Conference on Computer Vision and Pattern Recognition (CVPR), June, 2018.


% Planner Test
\bibitem{rare_event_sim} M. O\textquotesingle Kelly, A. Sinha, H. Namkoong, R. Tedrake, and J. C. Duchi, ``Scalable End-to-End Autonomous Vehicle Testing via Rare-event Simulation'', Advances in Neural Information Processing Systems 31, 2018, pp.9827--9838.

% RL
\bibitem{dde} Z.-W. Hong, T.-Y. Shann, S.-Y. Su, Y.-H. Chang, T.-J. Fu, and C.-Y. Lee, ``Diversity-Driven Exploration Strategy for Deep Reinforcement Learning'', Advances in Neural Information Processing Systems 31, 2018, pp.10489--10500.
\bibitem{svpg} Y. Liu, P. Ramachandran, Q. Liu, and J. Peng, ``Stein Variational Policy Gradient'', in Conference on Uncertainty in Artificial Intelligence (UAI), 2017
% Appeard in ICLR 2019
\bibitem{diayn} B. Eysenbach, A. Gupta, J. Ibarz, and S. Levine, ``Diversity is All You Need: Learning Diverse Skills without a Reward Function'', arXiv preprint arXiv:1802.06070, 2018.
% \bibitem{dqn} V. Mnih, K. Kavukcuoglu, D Silver, et al., ``Human-level control through deep reinforcement learning'', Nature 518, 2015, pp.529--533, doi:10.1038/nature14236.
\bibitem{chainerrl} Y. Fujita, T. Kataoka, P. Nagarajan, and T. Ishikawa, ``ChainerRL: A Deep Reinforcement Learning Library'', Deep Reinforcement Learning Workshop at Neural Information Processing Systems, 2019.  

\bibitem{pfn_sim} M. Miyashita, S. Maruyama, Y. Fujita, M. Kusumoto, T. Pfeiffer, E. Matsumoto, R. Okuta, and D. Okanohara, ``Toward Onboard Control System for Mobile Robots via Deep Reinforcement Learning'', Deep Reinforcement Learning Workshop at Neural Information Processing Systems, 2018.
\bibitem{intrinsic_reward_survey} A. Aubret, L. Matignon, and S. Hassas, ``A survey on intrinsic motivation in reinforcement learning'', arXiv preprint arXiv:1908.06976, 2019.

\end{thebibliography}
